SayDo: Benchmarking the Safety of Frontier Models from Chat to Closed-Loop Robot Control

Frontier vision-language models (VLMs) are increasingly used as high-level robot controllers, yet their safety is evaluated almost entirely in text. We introduce SayDo, a benchmark that assesses the propensity of frontier models to cause harm in embodied contexts. SayDo comprises eleven laboratory and household tasks that pair a benign instruction with a hazard latent in the scene. Tasks are implemented in six settings along an embodiment gradient, from chat questions about an imagined robot to closed-loop control of a simulated robot arm. Benign controls, safe-alternative variants and scripted operator pushback complement each task. Across six open- and closed-weight VLMs and 11,480 episodes, hazardous-action rates rise from 14% in chat to 47% in the simulator, and from 2% to 80% for the most affected model. The increase is largely driven by open-weight models. We find that models flag hazards before acting in 73% of unsafe episodes and give way to pushback about twice as often when controlling robots as in chat. The safest models also show signs of overcaution on benign controls. Safety evaluations run in text therefore do not predict the safety behavior of the same models when used as robot controllers.

==> generated-overview-rates.tex <==
\def\ovrateA{14}%
\def\ovrateB{13}%
\def\ovrateC{24}%
\def\ovrateD{32}%
\def\ovrateE{38}%
\def\ovrateF{47}%

